Maximum parsimony distance on phylogenetictrees: a linear kernel and constant factor approximation algorithm

Maximum parsimony distance is a measure used to quantify the dissimilarity of two unrooted phylogenetic trees. It is NP-hard to compute, and very few positive algorithmic results are known due to its complex combinatorial structure. Here we address this shortcoming by showing that the problem is fixed parameter tractable. We do this by establishing a linear kernel i.e., that after applying certain reduction rules the resulting instance has size that is bounded by a linear function of the distance. As powerful corollaries to this result we prove that the problem permits a polynomial-time constant-factor approximation algorithm; that the treewidth of a natural auxiliary graph structure encountered in phylogenetics is bounded by a function of the distance; and that the distance is within a constant factor of the size of a maximum agreement forest of the two trees, a well studied object in phylogenetics.

==> oldnotes.tex <==

\section{A constant-factor approximation algorithm (?)}

\textcolor{red}{It might be sensible in this section (and the corollary section) to use a symbol for the linear coefficient in the kernel bound. Otherwise the analysis will be tied to the specific number we derive in this paper: if we improve the bound (as we might before we submit), or future authors do, the analysis will be immediately outdated.}

This assumes that we have a \emph{linear} kernel.\\
\\
Something like this? \textcolor{red}{Note, for approximation purposes we should treat dMP as a maximization problem. Hence, we will need an upper bound relative to which we define the quality of our approximation algorithm. Probably the size of the actually realized kernel is the right upper bound to use?}

\begin{itemize}
    \item Apply the reduction rules; the \emph{size} of the kernel tells us something. But I don't think this is so useful; more useful is the fact that $d_{MP} \leq kernel size \leq f(d_{MP})$ for a linear function $f$. \textcolor{red}{On reflection, I do think the actual size of the kernel is important in the approximation algorithm.}
    \item Partition the first tree in polytime (c.f. Lemma \ref{cor:degreepartition}). \textcolor{red}{We need to decide how many blocks in the partition, this is the interesting bit: this will presumably be some function of the actually realised kernel size}.
    \item Use the partition to construct a character; run Fitch on the second tree; if the parsimony score on the second tree is large enough, we are done (just like in the kernelization argument)
    \item Otherwise, inspect an optimal extension (as produced by Fitch) and use that to extract a conflicting set of disjoint trees (just like in the kernelization argument).
    \item (Perhaps it is difficult to algorithmically decide which of the previous two cases holds: in which case we just do both and take the maximum?) \textcolor{red}{No, I no longer think this will be necessary}.
    \item This hopefully gives us a sufficiently good character. Reverse the reduction-rules to obtain a same or better quality character for the original trees (Lemma \ref{lem:backmap}).
\end{itemize}

\section{Easy corollaries}

\subsection{Bounding the distance between $d_{TBR}$ and $d_{MP}$}

\emph{Sketch}. It is well-known that $d_{MP} \leq d_{TBR}$. In several papers the question has been asked whether $d_{MP}$ can be arbitrarily small compared to $d_{TBR}$. We show that this is not the case, using the kernel argument earlier in the paper; specifically, we show that $d_{TBR}$ is at most a constant multiple of $d_{MP}$. After reducing common subtrees and shrinking chains to length 4, we obtain
a reduced pair of trees where both $d_{MP}$ and $d_{TBR}$ are preserved. If we let $t$ be the number of taxa in the reduced tree-pair, we get
\begin{equation}
d_{MP} \leq t \leq p \cdot d_{MP} 
\end{equation}
where $p$ is the bound on the $d_{MP}$ kernel size and
\begin{equation}
d_{MP} \leq d_{TBR} \leq t \leq q \cdot d_{TBR}
\end{equation}

where $q$ is the bound on the $d_{TBR}$ kernel size (currently $q=20$). Note that the inequalities $d_{MP} \leq t$ and $d_{TBR} \leq t$ follow from the trivial linear upper bounds on both the distances, as discussed in the preliminaries.\\
\\
Dividing the second inequality through by $d_{MP}$, and observing (from the first inequality) that $t \leq p \cdot d_{MP}$ holds, we obtain $1 \leq \frac{d_{TBR}}{d_{MP}} \leq p$.\\
\\
\textcolor{red}{Note that $q$ does not appear in the analysis. Maybe comment on this? Also, the two inequality chains might be useful in the approximation algorithm section, so consider introducing there.}

%----------------\\
%\\
%I think the claim that $d_{TBR} \leq f( d_{MP} )$ now follows from these two inequalities. See email discussion below, still needs to be formalized.

%\begin{verbatim}
%Hi Mark,

%I can't quite remember the exact bound on your kernel
%(I will re-read it a little later today before our call, but
%for the sake of argument let's say that you have proven that
%after kernelization, the following holds:
%
%|kernel| <= 2^dMP

%Now, we know that this kernelization presrves both
%dTBR and dMP, and that dTBR has a linear kernel, so we have

%|kernel| <= c.dTBR  (for some c that I can't be bothered to fill in)

%Noting that both dMP and dTBR are upper-bounded by |X|,
%and substituting the size of the kernel for |X|, we have

%log|kernel| <= dMP <= |kernel|                (1)

%(1/c)|kernel <= dTBR <= |kernel|              (2)

%This proves that TBR <= 2^dMP, or am I mistaken? If TBR > 2^dMP, then by (1)

%dTBR > 2^ [log|kernel|]
%      = |kernel|

%yielding contradiction on (2).
%\end{verbatim}


\subsection{A linear bound on the treewidth of display graphs}

Let $D$ be the display graph obtained by identifying those leaves of $T_1$, $T_2$ with the same label. It is known that $tw(D) \leq d_{TBR} + 2$.

Combining with the result from
the previous section, we obtain
$tw(D) \leq p \cdot d_{MP} + 2$.

This resolves an open question from X and Y. Interesting because Z.\\
\\
Note that Thm 7.2 of (treewidth distance on phylogenetic trees) shows a family of trees where tw=1 but $d_{MP}$ is unbounded.
